Self-Improved Retrosynthetic Planning

Retrosynthetic planning is a fundamental problem in chemistry for finding a pathway of reactions to synthesize a target molecule. Recently, search algorithms have shown promising results for solving this problem by using deep neural networks (DNNs) to expand their candidate solutions, i.e., adding new reactions to reaction pathways. However, the existing works on this line are suboptimal; the retrosynthetic planning problem requires the reaction pathways to be (a) represented by real-world reactions and (b) executable using "building block" molecules, yet the DNNs expand reaction pathways without fully incorporating such requirements. Motivated by this, we propose an end-to-end framework for directly training the DNNs towards generating reaction pathways with the desirable properties. Our main idea is based on a self-improving procedure that trains the model to imitate successful trajectories found by itself. We also propose a novel reaction augmentation scheme based on a forward reaction model. Our experiments demonstrate that our scheme significantly improves the success rate of solving the retrosynthetic problem from 86.84% to 96.32% while maintaining the performance of DNN for predicting valid reactions.

==> table/2_ablation_iter.tex <==
\begin{table*}[ht!]
\caption{Experimental results of our frameworks with multiple iterations. The above cell denotes the results of Retro*-0 + ours, and the below cell denotes the results of Retro*. As we repeat our procedure, we can further improve the multi-step retrosynthesis performance, whlie maintaining performance of single-step retrosynthesis.}
\label{tab:2_ablation_iter}
\vskip 0.15in
\begin{center}
\begin{sc}
\begin{tabular}{lc cc ccccc}
\toprule
& & \multicolumn{2}{c}{Single-step} & \multicolumn{5}{c}{Retrosynthetic planning} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-9}
Algorithm & Iter & Top-1 & Top-10 & \thead{Succ. rate \\ (N=50)} & \thead{Succ. rate \\ (N=500)} & \thead{Avg. \\ Length} & \thead{Avg. \\ Time} & \thead{Avg. \\ Cost} \\
\midrule
\multirow{3}{*}{Retro*-0 + Ours}  & 1    & 00.00 & 00.00 & 50.00 & 93.16 & 40.37 & 117.19  & 000  \\
                                & 2    & 00.00 & 00.00 & 52.11 & 95.26 & 30.20 & 104.37  & 000  \\
                                & 3    & 00.00 & 00.00 & 57.37 & 96.32 & 24.94 & 96.22  & 000  \\
\midrule
\multirow{3}{*}{Retro* + Ours}  & 1    & 00.00 & 00.00 & 51.58 & 90.00 & 55.75 & 122.18  & 000  \\
                                & 2    & 00.00 & 00.00 & 57.37 & 91.06 & 50.64 & 109.89  & 000  \\
                                & 3    & 00.00 & 00.00 & 00.00 & 00.00 & 00 & 000  & 000  \\
\bottomrule
\end{tabular}
\end{sc}
\end{center}
\vskip -0.1in
\end{table*}

==> trash/2_background_legacy.tex <==
\section{Background}
In this section, we state the problem we are tackling.
\subsection{Problem statement}
\textbf{Single-step retrosynthesis.}
Single-step retrosynthesis can be seen as a transformation from target molecule $t$ to set of $N$ reactant molecules $\{r_{i}\}_{i=1}^{N}$. In this paper, we ignore reagents and other chemical conditions following common practice. The goal of single-step retrosynthesis model is to predict a set of reactants $\{r_{i}\}_{i=1}^{N}$, which can be used to synthesize given target molecule $t$. 

% We denote single-step retrosyntheis model as $p(\mathcal{R} | m; \theta)$, where $\theta$ indicates parameter of the model.

%Single-step retrosynthesis can be seen as a transformation from target molecule $t$ to set of $N$ reactant molecules $\{R_{i}\}_{i=1}^{N}$. In this paper, we ignore reagents and other chemical conditions following common practice. The goal of single-step retrosynthesis model is to predict a set of reactants $\mathcal{R}$. which can be used to synthesize given target molecule $t$. We denote single-step retrosyntheis model as $p(\mathcal{R} | m; \theta)$, where $\theta$ indicates parameter of the model.

% They have shown promising results, but use atom-mapping information between products and reactants as an additional type of supervision.


% In the DNN-based approaches, the DNN is trained to predict $\mathcal{R}$ given target molecule $t$ using a dataset $\mathcal{D}_{train} = \{t_{i}, \mathcal{R}_{i} \}$.\footnote{reagents and and other chemical reaction conditions are ignored for simplicity following common practice.} The 


% The single-step retrosynthesis model is trained using a dataset $\mathcal{D}_{train} = \{t_{i}, \mathcal{R}_{i} \}$ in common.\footnote{reagents and and other chemical reaction conditions are ignored for simplicity following common practice.}


\textbf{Retrosynthetic planning.}
{
\color{blue}
In retrosynthetic planning, we aim to construct a reaction pathway for synthesizing a target molecule $t \in \mathcal{M}$ using building-block molecules $\mathcal{I} \subset \mathcal{M}$ that are accessible to chemists, e.g., a set of commercially available molecules. Throughout the paper, we represent each retrosynthetic route $\tau = \{R_{k}\}_{k=1}^{M}$ as a set of reactions. Each reaction $R=(m, \{r_{i}\}_{i=1}^{N})$ is represented by the corresponding product $m$ and reactants $\{r_{i}\}_{i=1}^{N}$. We say that a retrosynthetic route $\tau$ is a \textit{success route} if the retrosynthetic route correctly maps the target molecule into a set of building blocks.

In this work, we say that the retrosynthetic direction (from $m$ to $\mathcal{R}$) is \textit{backward}, and the synthetic direction (from $\mathcal{R}$ to $m$) is \textit{forward}, where $\mathcal{R}=\{r_{i}\}_{i=1}^{N}$. We consider a single-step backward model $p_{\theta_{b}}(\mathcal{R}|m)$ that aims to find a set of reactants that aims to find a set of reactants $\mathcal{R}$ for synthesizing the product $m$. A single-step forward model $p_{\theta_{f}}(m|\mathcal{R})$ predicts product $m$ given a set of reactants $\mathcal{R}$. We denote search algorithm as $\pi_{\theta_{b}}$, where $\theta_{b}$ is the parameter of the single-step backward model which is utilized to expanding candidates.
}
% In retrosynthetic planning, we aim to find a series of reactions which is able to transform a given single target molecule $t \in \mathcal{M}$ into a set of building-block molecules $\mathcal{I} \subset \mathcal{M}$, i.e., a set of commercially available molecules. Throughout the paper, we denote retrosynthetic route as a series of set of molecules $\tau_{t} = \{\mathcal{M}_{1}^{t}, \mathcal{M}_{2}^{t}, \ldots, \mathcal{M}_{K}^{t} \}$, where $t$ is a target molecule, and $M_{k}^{t}$ is a set of intermediate molecules which are transformed from the target molecule $t$. We say $\tau_{t}$ is a \textit{success route} if the last set of molecules is a subset of building-block molecules $\mathcal{I}$, i.e., $\mathcal{M}_{K}^{t} \subset \mathcal{I}$. 

{
\color{red}
In retrosynthetic planning, we aim to construct a reaction pathway for synthesizing a target molecule $t \in \mathcal{M}$ using building-block molecules $\mathcal{I} \subset \mathcal{M}$ that are accessible to the chemist, e.g., a set of commercially available molecules. Throughout the paper, we represent each synthetic route $\tau = \{R_{k}\}_{k=1}^{M}$ as a set of reactions. Each reaction $R=(m, \{r_{i}\}_{i=1}^{N})$ is represented by the corresponding product $m$ and reactants $\{r_{i}\}_{i=1}^{N}$. We say that a synthetic route $\tau$ is a success route if the synthetic route correctly maps a set of building blocks into the target molecule. 
}

{
\color{red}
In this work, we consider a single-step retrosynthesis model $p_{\theta}(\mathcal{R}|m)$ that aims to find a set of reactants $\mathcal{R}=\{r_{i}\}_{i=1}^{N}$ for synthesizing the product $m$. 
}


% A reaction $A_{i}$ transforms given set of molecules $\mathcal{R}_{i}$ into $\mathcal{R}_{i+1}$, and we denote $\mathcal{R}_{i+1} = A_{i}(\mathcal{R}_{i})$. In this paper, we say $\mathcal{A}_{t}$ is a \textit{success route} if $t$ can be successfully transformed into a set of building-block molecules by applying the reactions $A_{k}$ in order, i.e., $A_{|\mathcal{A}_{t}|} \circ A_{|\mathcal{A}_{t}|-1} \circ \ldots \circ A_{1}(t) = \mathcal{R}_{|\mathcal{A}_{t}|} \subset \mathcal{I}$.

% Recent works on retrosynthetic planning focus on developing search algorithms by expanding candidate solutions using trained single-step model\cite{segler2018planning, kishimoto2019depth, chen2020retro}. For example, \citet{segler2018planning} employed Monte Carlo Tree Search (MCTS) for retrosynthetic planning. \citet{kishimoto2019depth, chen2020retro} developed search algorithm based on AND/OR tree utilizing proof number search and A* search, respectively. We denote retrosynthetic search algorithm as $\pi_{\theta}$, where $\theta$ is the parameter of the single-step retrosynthesis model $p(\mathcal{R} | m; \theta)$.



==> trash/2_related_legacy.tex <==
\section{Related Works}
In general, retrosynthetic planning is solved by updating intermediate synthetic routes in a reverse order, i.e., adding product to intermediate synthetic routes before its reactants. To this end, a  \textit{single-step retrosynthetic model} iteratively propose a set of reactants to synthesize a product in a candidate synthetic route. The data structure and the protocol of updating the intermediate synthetic routes are determined by a \textit{search algorithm} that prioritizes on finding a highly-rewarding solution with small number of updates. 

%The choice of product being analyzed by the single-step retrosynthetic model is specific to the search algorithm, e.g., 
%At each iteration, the algorithm expands 
%starting from a target molecule. At each iteration, the algorithm expands its tree by choosing a molecule and proposing a set of reactants to synthethize it using a \textit{single-step retrosynthetic model}. 
%``working backwards,'' analysing molecules recursively and transforming them into simple precursors until one obtains a set of known or commercially available building-block molecules. To this end, a 
%The main challenge is twofold. First, one should use an accurate \textit{single-step retrosynthetic model} that provides the desired proposals for expanding a node in the search tree. For example, each expansion of a node should represent a realistic reaction for synthesizing the target product. Next, nodes that are expanded should be chosen smartly. This is done by a \textit{search algorithm} to maximize the reward from the found trajectory.
%These programs select among possible reactions using heuristic scoring functions, \citep{xx}, crowd-sourced accessibility scores, \citep{xx} analogy to precedent reactions \citep{xx}. 
%To solve retrosynthetic planning, 
%Retrosynthetic planning is a fundamental problem in chemistry for finding a pathway of reactions to synthesize a target moelcule. 
%To achieve this, Prior reports on retrosynthetic planning have explored a variety of policies for guiding the generation of candidate syntheses. These programs select among possible reactions using heuristic scoring functions, [7, 15] crowd-sourced accessibility scores, [13, 16] analogy to precedent reactions, [17]. 
%In particular, deep neural networks have recently emerged as  

\textbf{Single-step retrosynthetic model.}
Researchers have studied various computational methods to propose a set of reactants for synthesizing the given product, e.g., heuristic scoring functions \citep{xx}, crowd-sourced accessibility scores \citep{xx}, and analogy to precedent reactions \citep{xx}. Especially, recent works have shown promising results based on a deep neural network that propose reactant sets given the product as its input. Such works commonly assume a real-world dataset for training and evaluating the single-step retrosynthetic model based on supervised learning. Exceptionally, \citet{schreck2019learning} considered reinforcement learning for training its single-step retrosynthetic model to propose reactants that are likely to generate synthetic routes with low cost for execution. 

%They are mainly categorized into template-based \citep{xx} or template-free methods \citep{xx}, depending on their reliance on the reaction templates, i.e., subgraph patterns describing how the chemical reaction occurs among reactants. These works assume the existence of 

%Recently, computational methods for single-step retrosynthesis has shown promising results \cite{coley2017computer, segler2017neural, dai2019retrosynthesis, liu2017retrosynthetic, karpov2019transformer, zheng2019predicting, shi2020graph, somnath2020learning, yan2020retroxpert}. They are mainly categorized into template-based or template-free methods, depending on their reliance on the reaction templates, i.e., subgraph patterns describing how the chemical reaction occurs among reactants. The templates can be hand-crafted by experts \cite{hartenfeller2011collection, szymkuc2016computer}, or extracted algorithmically from reaction databases \cite{law2009route, coley2017prediction}. The template-based approaches aim to learn prioritizing templates to apply into given target molecule. Despite their chemical interpretability, they lack generalization to new reactions. Template-free methods \cite{liu2017retrosynthetic, karpov2019transformer, zheng2019predicting, shi2020graph, somnath2020learning, yan2020retroxpert} generate the reactants from scratch, avoiding reliance on the templates. \citet{liu2017retrosynthetic, karpov2019transformer, zheng2019predicting} formulate single-step retrosynthesis as a conditional generation problem such as machine translation. Another line of works in template-free methods is based on synthon generation, which is incomplete molecule between product and reactants \cite{shi2020graph, somnath2020learning, yan2020retroxpert}. They decompose retrosynthesis prediction into two tasks: i) breaking down given target molecule into a set of synthons; and ii) expanding the synthons into reactants. 

\textbf{Search algorithms.}
Since the number of synthetic routes proposed by a single-step retrosynthetic model can be exponentially large, researchers applied search algorithms to guide the generation of synthetic routes. Existing search algorithms such as Monte Carlo tree search \cite{segler2018planning}, and proof number search \cite{kishimoto2019depth} have been used. Notably, \citet{chen2020retro} developed a search algorithm specific to the A* search \citep{xx} specifically for the retrosynthetic planning problem.  

%To find success route of the target molecule, commonly used method is performing  backward chaining that starts from the target molecule, instead of performing forward chaining which starts from $\mathcal{I}$ \cite{segler2018planning, schreck2019learning, kishimoto2019depth, chen2020retro}. They search success route using planning algorithms such as Monte Carlo Tree Search (MCTS) \cite{segler2018planning}, Greedy search \cite{schreck2019learning}, Proof number search \cite{kishimoto2019depth}, or A* search \cite{chen2020retro}, expanding candidate reactions using single-step model. The planning algorithms are usually guided by value function, which estimates cost to synthesize a molecule. The value function can be designed heuristically \cite{kishimoto2019depth}, or trained by using true success routes \cite{chen2020retro}, or simulated routes \cite{segler2018planning, schreck2019learning}.



%\section{Related works}
%Recent deep learning based approaches on retrosynthetic planning usually decompose the task into (i) training single-step %retrosynthesis model and (ii) developing search algorithms utilizing the trained single-step retrosynthesis model in a %iterative manner.
%
%\textbf{Single-step retrosynthesis.}
%The goal of single-step retrosynthesis is to train a model which predicts direct reactants given target molecule. Existing %methods are roughly categorized into template-based or template-free. Templates are subgraph pattern rewriting rules, which %are either encoded by experts \cite{hartenfeller2011collection, szymkuc2016computer} or extracted from reaction database %\cite{law2009route, coley2017prediction}. Template-based methods prioritize templates which match given target molecule.
%
%% by either similarity between the target and templates \cite{coley2017computer} or 
%
%
%Template-free methods \cite{liu2017retrosynthetic, karpov2019transformer, zheng2019predicting, shi2020graph, %somnath2020learning, yan2020retroxpert} generate the reactants from scratch, avoiding reliance on the templates. %\citet{liu2017retrosynthetic, karpov2019transformer, zheng2019predicting} regard single-step retrosynthesis as a conditional %generation problem such as machine translation. Another line of works in template-free methods is based on decomposition of %retrosynthesis prediction into two tasks: i) breaking down given target molecule into a set of incomplete molecules called %synthons; and ii) expanding synthons into reactants \cite{shi2020graph, somnath2020learning, yan2020retroxpert}. They have %shown promising results, but use atom-mapping information between products and reactants as an additional type of supervision.
%
%% \citep{shi2020graph, somnath2020learning, yan2020retroxpert} has shown promising results by decomposing retrosynthesis %prediction into two tasks: i) breaking down given target molecule into a set of incomplete molecules called synthons; and ii) %expanding synthons into reactants. However, they need atom-mapping between products and reactants as an additional %supervision.
%
%\textbf{Search algorithms of retrosynthetic planning.}
%\citet{segler2018planning, kishimoto2019depth, chen2020retro} aim at developing search algorithms, relying on fixed %single-step model. \citet{segler2018planning} employed Monte Carlo Tree Search (MCTS) for retrosynthetic planning. %\citet{kishimoto2019depth, chen2020retro} developed search algorithm based on AND/OR tree utilizing proof number search and A* %search, respectively.
%
%
%% MCTS consists of four steps: i) Selection of the most promising leaf node in current search tree, ii) Expansion of the tree %using single-step retrosynthesis at the selected node. iii) Evaluation of the new node using rollout. iv) Update of 


==> trash/3_method.tex <==
\section{Self-improving procedure of single-step retrosynthesis}
\input{algorithm/algo}
\subsection{Overview}
In this section, we introduce a new framework for training the single-step model towards expanding the retrosynthetic routes in a direction that is realistic and executable from building block molecules. Our main idea is based on self-improving procedure, which trains the single-step model to imitate pathway found by itself combined with existing search algorithms. We also propose new augmentation method based on domain knowledge in chemistry, using single-step forward model and the generated pathways. Dataset $\mathcal{D}$ stores targets which the single-step backward model to imitate.

% Multi-step algorithm, which use the improved single-step model as a submodule, can find more success routes within a  shorter time.

% \textst{To apply our framework, we view the single-step retrosynthesis as Markov decision process, which is defined as a tuple $(\mathcal{S}, \mathcal{A}, \mathcal{P}, r)$. Here, $\mathcal{S}$ is the state space, $\mathcal{A}$ is the action space, $\mathcal{P}(s'|s,a)$ is the transition dynamics, $r(s,a)$ is the reward function. In our setting, state $s \in \mathcal{S}$ is a molecule, and action $a \in \mathcal{A}$ is a single-step retrosynthetic reaction. The transition matrix $\mathcal{P}(s'|s,a)$ is probability distribution over next state $s'$ given current state $s$ and action $a$. In our setting, $\mathcal{P}(s'|s,a) = \frac{1}{|\mathcal{R}|} \mathds{1}(s' \in \mathcal{R})$ where $\mathcal{R}$ is a set of reactant, which is generated by applying single-step retrosynthetic reaction $a$ into molecule $s$. $\mathds{1}$ denotes the indicator function that takes the value 1 if the condition is satisfied, and 0 otherwise.}

% The single-step retrosynthesis model can be viewed as an apprentice policy $p_{\theta}(a|s)$, which is a probability distribution over all actions $a$ given state $s$. We denote expert policy as $\pi(a|s; p_{\theta})$, which generates target demonstrations for apprentice policy $p_{\theta}$ to imitate. Search algorithm combined with the single-step retrosynthesis model can be used as an expert policy $\pi$.
% which state $s$ is a molecule and action $a$ is a single-step reaction to apply.

% Throughout the paper, we say that the retrosynthetic direction (from $P$ to  $\mathcal{R}$) is \textit{backward}, and the synthetic direction (from $\mathcal{R}$ to $P$) is \textit{forward}. We denote single-step backward model as $p(\mathcal{R} | m ; \theta_{b})$, and single-step forward model as $p(m | \mathcal{R}; \theta_{f}))$. Retrosynthetic planning algorithm, utilizing the single step model $p(\cdot | m; \theta_{b})$ for expanding candidates, is denoted as $\pi_{\theta_{b}}$. 

Our framework iterates the following procedure:
\begin{itemize}
    \item \textbf{Step A.} Sample target molecule and generate retrosynthetic success route using the retrosynthetic planning algorithm.
    \item \textbf{Step B.} Extract demonstrations, which are single-step reactions, from the success route.
    \item \textbf{Step C.} Augment demonstrations from the extracted demonstrations using pre-trained single-step forward model, and store all the demonstrations into dataset $\mathcal{D}$.
    \item \textbf{Step D.} Train a single-step backward model with imitation learning using the dataset $\mathcal{D}$.
\end{itemize}

\comment{
Our framework iterates the following procedure:
\begin{itemize}
    \item \textbf{Step A.} Sample target molecule $m_{1} \sim \mathcal{T}$ and generate retrosynthetic route $\tau_{t} = \{ \mathcal{M}_{k}^{t}\}_{k=1}^{K}$ from $t$ from retrosynthetic planning algorithm $\pi_{\theta_{b}}$.
    \item \textbf{Step B.} Extract demonstrations, which are tuple of (molecule, reactants, score) $\{m_{k}, \mathcal{R}_{k}, \phi(m_{k}, \mathcal{R}_{k})\}_{k=1}^{K}$ from route $\mathcal{A}_{t}$ into dataset $\mathcal{D}$.
    \item \textbf{Step C.} Generated augmented demonstration $\{m'_{k}, \mathcal{R}_{k}, \phi(m'_{k}, \mathcal{R}_{k})\}_{k=1}^{K}$ using single-step forward model $p(m | \mathcal{R}; \theta_{f})$ and $\{m_{k}, \mathcal{R}_{k}, \phi(m_{k}, \mathcal{R}_{k})\}_{k=1}^{K}$
    \item \textbf{Step D.} Train single-step model $p(\mathcal{R}|m; \theta)$ with imitation learning using dataset $\mathcal{D}$
\end{itemize}
}

One can note that our framework resembles prior works on expert iteration \cite{anthony2017thinking, anthony2019policy} and AlphaGo Zero \cite{silver2017mastering}, where Monte Carlo tree search is regarded as a stronger operator that guides training neural network. Reactions in success routes can be seen as expert demonstrations. Comparing to the prior works, we use additional expert, the single-step forward model which augment expert demonstrations. By imitating expert demonstrations, single-step backward model can be trained to generate reactions which are realistic and executable from building blocks. We provide an illustration and a detailed description of our algorithm in Figure \textcolor{red}{X} and Algorithm \ref{alg:algo}, respectively.

\subsection{Generating Expert Demonstrations}
In this section, we provide a detailed description of generating expert demonstrations, which are targets for single-step backward model to imitate. At first, we sample a target molecule $t$ from molecule dataset $\mathcal{T}$. Then, we generate retrosynthetic route $\tau_{t} = \{R_{k}\}_{k=1}^{M}$ from retrosynthetic planning algorithm $\pi_{\theta_{b}}$. Then we extract expert demonstration $\{m_{k}, \mathcal{R}_{k} \}_{k=1}^{K}$ from the route $\tau_{t}$. We can further augment the expert demonstrations using single-step forward model. The detailed descriptions are as follows.
% Then, we predict retrosynthetic reaction $a$ using expert policy $\pi(a|s; p_{\theta})$
%Then, we generate trajectory $\tau = (s_{0}, a_{0}, s_{1}, a_{1}, \ldots, s_{T})$ from expert policy $\pi(a|s; p_{\theta}(a|s))$. 
% Then, we extract all the state-action pairs $(s_{t}, a_{t})$ and add the pair with the corresponding score $\phi(s,a)$ into dataset $\mathcal{D}$.

\textbf{Generating success routes.}
At first, we sample a target molecule $t$ from target molecule dataset $\mathcal{T}$. Then we run retrosynthetic planning algorithm $\pi_{\theta_{b}}$ until a success route $\tau_{t}$ is found under a limit of the number of expansions. If success route for the target molecule $t$ is not found, we ignore the target molecule and the corresponding incomplete routes. Any retorsynthetic planning algorithm can be used for our framework. We use Retro*-0 and Retro* \cite{chen2020retro} as retrosynthetic planning algorithms, which have shown the best performance in the field of retrosynthetic planning.

% We propose two types of experts: (1) oracle and (2) retrosynthetic planning algorithms. Firstly, the demonstrations from oracle can be seen as hand-coded success routes by chemists. We regard given success routes as demonstrations from oracle. Secondly, inspired by the prior works on expert iteration \cite{anthony2017thinking, anthony2019policy} and AlphaGo Zero \cite{silver2017mastering}, multi-step retrosynthesis planner can be seen as an expert.


\textbf{Extracting expert demonstrations.}
From the generated success route $\tau_{t}$, we extract expert demonstrations, that are single-step reactions. At first, we collect all the single-step reactions $R_{k}$ in the success route $\{R_{k}\}_{k=1}^{M}$. Then, we filter out reactions which are invalid in the view of single-step retrosynthesis. However, there can be unrealistic single-step reaction in the success route, and using this noisy demonstrations for imitation learning show performance degradation in single-step retrosynthesis model. To alleviate this, we filter out unrealistic single-step demonstrations using likelihood under pre-trained single-step retrosynthesis model. This filtering scheme shows its effectiveness in our experiments.


% We design score function which measure quality of each demonstration. We calculate the score by considering two criteria simultaneously: (1) demonstration is from success route, and (2) the cost of demonstration is under threshold $\delta$. The cost is user-defined value, i.e., price of the reaction, or the negative log-likelihood the reaction under single-step retrosynthesis model. We use the negative log-likelihood under pretrained single-step retrosynthesis model for the cost. The score function is designed as follows:

\comment{
\begin{equation*}\label{eq:score}
\begin{aligned}
    \phi(m, \mathcal{R}) = \mathds{1}[(m, \mathcal{R}) \;is \;from \;success \;route \;and \\
    \;\mathtt{cost}(m, \mathcal{R}) < \delta]
\end{aligned}
\end{equation*}
}

\textbf{Augmenting expert demonstrations.}
We propose new augmentation scheme based on domain knowledge in chemistry, which generate additional expert demonstrations using pre-trained single-step forward model and the extracted demonstrations. We note that there can be multiple valid products from same reactants depending on various chemical conditions \citep{xx}. Based on this knowledge, we can generate a \textit{pseudo-product} $m'$, which is predicted product from the pre-trained single-step forward model $p_{\theta_{f}}(\cdot | \mathcal{R})$. Then, we can obtain additional single-step reaction. Then, we can obtain additional single-step reaction $\{m'_{k}, \mathcal{R}_{k}\}_{k=1}^{K}$ from the extracted reactions $\{m_{k}, \mathcal{R}_{k}\}_{k=1}^{K}$. The pseudo-product $m'$ can be either same with or different from the original product $m$. We do not remove augmented single-step reaction $\{m'_{k}, \mathcal{R}_{k}\}$ which pseudo-product is same with the original product, as it means that the reaction is strongly realistic. Maintaining the duplicated reactions can help to train single-step retrosynthesis model learn valid reactions. We note that unrealistic products can be generated from the forward model. To avoid generate single-step reactions that are invalid, we filter out unrealistic reactions utilizing pre-trained single-step retrosynthesis model. We filter out augmented single-step reaction which do not satisfy $\mathcal{R}_{k} = \argmax_{\mathcal{R}} p_{\theta_{b}}(\mathcal{R} | m'_{k})$. Throughout this augmentation, we can obtain augmented single-step reactions which are realistic and executable from building blocks.


\subsection{Imitation Learning}
Finally, we describe our learning scheme for training single-step backward model using the generated expert demonstrations $\mathcal{D}$.
We adopt Behavioral Cloning (BC) \cite{pomerleau1991efficient} as an imitation learning algorithm. BC trains apprentice policy $p_{\theta}$ by mimicking the expert demonstrations $\mathcal{D}$. The objective of BC in common is as follows:
\begin{equation*}\label{eq:bc}
    \argmax_{\theta_{b}} \mathbb{E}_{(m, \mathcal{R}) \in \mathcal{D}} [\log p_{\theta_{b}} (\mathcal{R} | m)],
\end{equation*}

% However, there can be demonstrations which have high cost, though the corresponding route ends up in building blocks. Using these demonstrations may harm to performance of single-step model. To alleviate the side-effect, utilizing the score which describe the quality of demonstration showed effectiveness. We weighted each demonstration with the designed score function $\phi$. Then, the objective becomes:
\comment{
\begin{equation*}\label{eq:bc}
    \argmax_{\theta} \mathbb{E}_{(m,\mathcal{R}, \phi(m,\mathcal{R})) \in \mathcal{D}} [\log p_{\theta} (\mathcal{R} | m; \theta) \cdot \phi(m,\mathcal{R})],
\end{equation*}
}
We can train the single-step backward model to generate reaction which is realistic and executable from building-blocks by imitating demonstrations from experts. 

After imitation learning, we can iterate the whole procedure with the updated single-step retrosynthesis model. Then, we can further train the single-step backward model to generate reaction which is realistic and executable from building blocks.



% One may also interpret this as filtering out noisy expert demonstrations using confidence score of single-step retrosynthesis model.

% One may also interpret this as BC with imperfect demonstrations \cite{wu2019imitation}, where gives sample weights based on confidence score.

% One can interpret the objective as training single-step model to imitate extracted single-step reactions from success routes generated by itself combined with search algorithms.

==> trash/4_ablation_delta.tex <==
\begin{table}[h]
\caption{Top-$k$ exact match accuracy \% under different filtering with different threshold in our framework. Measured at validation USPTO reaction dataset. Thr denotes threshold.}
\label{tab:2_ablation_delta}
\vskip 0.15in
\begin{center}

\begin{small}
\begin{sc}
\begin{tabular}{l ccccc}
\toprule
& \multicolumn{5}{c}{Single-step} \\
\cmidrule(lr){2-6}
Thr & Top-1 & Top-2 & Top-3 & Top-5 & Top-10\\
\midrule
0.9    & 44.42 & 56.97 & 62.72 & 68.21 & 72.45 \\
0.8    & 44.53 & 56.96 & 62.74 & 68.20 & 72.40 \\
0.7    & 44.52 & 56.94 & 62.74 & 68.16 & 72.40 \\
0.6    & 44.51 & 56.89 & 62.67 & 68.12 & 72.37 \\
0.5    & 44.48 & 56.83 & 62.65 & 68.08 & 72.36 \\
0      & 40.98 & 53.42 & 59.68 & 65.93 & 70.92 \\


\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
